TopiOCQA: Open-domain Conversational Question Answering with Topic Switching

In a conversational question answering scenario, a questioner seeks to extract information about a topic through a series of interdependent questions and answers. As the conversation progresses, they may switch to related topics, a phenomenon commonly observed in information-seeking search sessions. However, current datasets for conversational question answering are limiting in two ways: 1) they do not contain topic switches; and 2) they assume the reference text for the conversation is given, i.e., the setting is not open-domain. We introduce TopiOCQA (pronounced Tapioca), an open-domain conversational dataset with topic switches on Wikipedia. TopiOCQA contains 3,920 conversations with information-seeking questions and free-form answers. On average, a conversation in our dataset spans 13 question-answer turns and involves four topics (documents). TopiOCQA poses a challenging test-bed for models, where efficient retrieval is required on multiple turns of the same conversation, in conjunction with constructing valid responses using conversational history. We evaluate several baselines, by combining state-of-the-art document retrieval methods with neural reader models. Our best model achieves F1 of 55.8, falling short of human performance by 14.2 points, indicating the difficulty of our dataset. Our dataset and code is available at https://mcgill-nlp.github.io/topiocqa

==> figures/human_annotation.tex <==
\begin{figure}[]
\includegraphics[]{figures/files/human_annotation_column.png}
\caption{} 
\label{fig:topic-heatmap}
\end{figure}

==> tables/answer_analysis.tex <==
% \begin{table}[h]

% \centering
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{lc}
% \toprule
% Answerable
% & 7.9\%\\
% \midrule
% Span Found
% & 0.00\%\\
% \midrule
% Named Entity
% & 34.1\%\\
% Noun Phrase
% & 4.5\%\\
% Yes
% & 10.2\%\\
% No
% & 1.0\%\\
% Number
% & 3.6\%\\
% Date/Time
% & 6.0\%\\
% Other
% & 40.6\%\\
% \bottomrule
% \end{tabular}
% % }

% \caption{Answer statistics of \shortname{}}
% \label{tab:answer-analysis}
% \end{table}

\begin{table}[t]

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l r r r}
\toprule
& CoQA  & QReCC & \shortname{}\\
\midrule
Unanswerable & 1.3\% & 8.7\% & 7.9\%\\
% \midrule
Span found & 66.8\% & 39.28\% & 40.1\%\\
% 40.58 for QReCC test set
Avg. F1 of Best Span Match & 97.8 & 86.11 & 85.77 \\
Avg. answer length & 2.7 & 18.7 & 11.8\\
\bottomrule
% Noun Phrase & 67.6\% & 98.9\% & 94.0\% \\
% Verb Phrase & 15.5\% & 86.7\% & 44.0\% \\
% Named Entity & 33.8\% & 92.1\% & 72.8\% \\
% Yes & 11.0\% & 0.6\% & 10.6\% \\
% No & 8.6\% & 0.5\% & 1.0\% \\
% Number & 13.1\% & 47.8\% & 22.0\% \\
% Date/Time & 4.2\% & 31.7\% & 11.5\% \\
% Other & 18.1\% & 86.1\% & 38.6\% \\
\end{tabular}
}

\caption{Answer statistics of CoQA, QReCC and \shortname{}}
% \srcomment{These numbers do not add up to 100\%. I don't understand how you can have 94\% noun phrases and at the same time 44\% verb phrases}
\label{tab:answer-analysis}
\end{table}

==> tables/bias_exploit_results.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\centering {\begin{tabular}{lcccccccc}
\toprule       
Model & Question Rep & \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\ 
\cmidrule(r){3-5} \cmidrule(r){6-8}

& & EM & F1 & BLEU & EM & F1 & BLEU \\

\midrule
& Original
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
BM25 + DPR Reader & All history
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& T5 re-write
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\midrule

& Original
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
BM25 + FiD & All history
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& T5 re-write
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\midrule

& Original
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
DPR Retriever + DPR Reader & All history
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& T5 re-write
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\midrule

& Original
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
DPR Retriever + FiD & All history
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& T5 re-write
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\bottomrule
\end{tabular}}}
% }
\caption{Overall performance of all model variants on \shortname{} dev and test set, using the boosted scores of likely passages.}
\label{tab:bias-exploit-results-table}
\end{table*}


==> tables/qr_results.tex <==
\begin{table}[]

\centering {\begin{tabular}{lcc}
\toprule       
Model & ROGUE & BLEU \\ 

\midrule                         
Transformer++
& 00.00 & 00.00 \\
T5
& 00.00 & 00.00 \\

\bottomrule
\end{tabular}}
% }
\caption{Performance of T5 and Transformer++ on QReCC}
\label{tab:qr-table}
\end{table}

